Systemic Risk in Financial Networks: A Survey

We provide an overview of the relationship between financial networks and systemic risk. We present a taxonomy of different types of systemic risk, differentiating between direct externalities between financial organizations (e.g., defaults, correlated portfolios and firesales), and perceptions and feedback effects (e.g., bank runs, credit freezes). We also discuss optimal regulation and bailouts, measurements of systemic risk and financial centrality, choices by banks' regarding their portfolios and partnerships, and the changing nature of financial networks.

==> cycles.tikz.tex <==
\begin{tikzpicture}[scale=0.8]
\foreach \Point/\PointLabel/\location in {(0,0)/1, (3,3)/2, (6,0)/3, (3,-3)/4}
\draw[fill=black!20]  \Point circle (0.35) node {$\PointLabel$};
\draw[->, thick] (0,0.7) to [out=90,in=180] (2.3,3);
\draw[->, thick] (3.7,3) to [out=0,in=90] (6,0.7);
\draw[->, thick] (6,-0.7) to [out=-90,in=0] (3.7,-3);
\draw[->, thick] (2.3,-3) to [out=180,in=-90] (0,-0.7);

\draw (0,2.5) node {\small$15$}; \draw (6,2.5) node {\small$20$}; \draw (6,-2.5) node {\small$15$}; \draw (0,-2.5) node {\small$25$};

\foreach \Point/\PointLabel/\location in {(12,0)/1/left, (15,3)/2/above, (18,0)/3/right, (15,-3)/4/below}
\draw[fill=black!20]  \Point circle (0.35) node {$\PointLabel$};
\draw[->, thick] (15.7,3) to [out=0,in=90] (18,0.7);
\draw[->, thick] (14.3,-3) to [out=180,in=-90] (12,-0.7);

\draw (18,2.5) node {\small$5$}; \draw (12,-2.5) node {\small$10$};

  \end{tikzpicture}  

==> impossibility_example.tikz.tex <==
\begin{tikzpicture}[scale=8]

\foreach \Point/\PointLabel in {(1,0)/1, (4,0)/4}
\draw[fill=magenta!50] \Point circle (0.35) node {$\PointLabel$};
\foreach \Point/\PointLabel in {(6,3)/2, (6,-3)/3, (-3,-3)/5, (-3,3)/6}
\draw[fill=cyan!50] \Point circle (0.35) node {$\PointLabel$};


\draw[->, thick] (1.1,0.5) to [out=70,in=180] node [ above, sloped]  {$\frac{3D}{4}$} (5.5,3);
\draw[->, thick] (6.4,2.7) to [out=-50,in=50] node [ above, sloped]  {$D$}  (6.4,-2.7);
\draw[->, thick] (5.5,-3) to [out=180,in=-70] node [ below, sloped]  {$\frac{D}{2}$} (1.1,-0.5);
\draw[->, thick] (0.9,0.5) to [out=110,in=0] node [ above, sloped]  {$\frac{D}{2}$} (-2.5,3);
\draw[->, thick] (-2.5,-3) to [out=0,in=-110] node [ below, sloped]  {$\frac{D}{2}$} (0.9,-0.5);

\draw[<-, thick] (4.4,0.4) to node [ below, sloped]  {$\frac{D}{2}$} (6,2.5);
\draw[->, thick] (4,0.5) to node [ above, sloped]  {$\frac{D}{2}$} (5.6,2.6);
\draw[<-, thick] (4.4,-0.4) to node [ above, sloped]  {$\frac{D}{2}$} (6,-2.5);
\draw[->, thick] (4,-0.5) to node [ below, sloped]  {$\frac{3D}{4}$} (5.6,-2.6);

  \end{tikzpicture}  
